New Results For the Five Point Function

We present the new results of the computed general five-point functionby the magic spinor product method in loop integrals proposed by one (BFLW) of us. The result from the magic spinor product method agrees with that from LoopTools overall. Such encouraging agreements indicate that the magic spinor product method is a reliable approach with good efficiency and numerical stability.

==> axodraw2/INSTALL <==
MANUAL INSTALLATION of axohelp v. 1.2 and axodraw2
==================================================



A. Fully Manual Installation
----------------------------

   Note: if you do not wish to use axodraw2 with pdflatex, xelatex, or
         lualatex, but will only use it with latex, then only the
         first step is needed.

  1.  Copy axodraw2.sty to a suitable directory for LaTeX style files.

  2.  Compile the axohelp program by a command line like

          gcc -o axohelp -Wall -O3 axohelp.c

      (The exact details of the command line depend on your operating
      system and which compiler you have installed for the C
      language.)

  3.  Move axohelp to a suitable directory for executables.

  4.  (Optional) Copy axodraw2-man.pdf to a suitable directory for
                 LaTex package documentation.

  5.  (Optional) Copy axohelp.1 to a suitable directory for man pages.
  

B. Using autoconf etc:
---------------------

   You can also make axohelp using the GNU utilities autoconf,
   automake and autoreconf (if these are installed).  Doing this is
   enormous overkill for a program like axohelp with a single source
   file and with no need to make adjustments dependent on the
   operating system etc. Even so, we provide the files necessary for
   the use of autoconf and automake, since these are needed when the
   axodraw2 package is incorporated into TeXLive (which has an
   enormous automated build process).  So here are the instructions
   for building with autoconf and automake.  For these, it is assumed
   that the GNU utilities autoconf, automake and autoreconf are
   installed:

   As in Fully Manual Installation, but replace step 2 by

  2'. Run

      autoreconf --install
     ./configure
     make

  Note that there are a couple of test scripts: axohelp.test, which
  gives a rudimentary test, and axohelp-big.test, which gives a
  comprehensive test on all axodraw2 objects used in the
  manual. **Warnings**: a. You could get a spurious failure of a test
  because of a mismatch between the line-endings of the test file and
  the file generated by axohelp (UNIX \n v. MS-Windows \r\n).  b. You
  could also get spurious test failure because of differences in the
  effects of rounding error with your compiled axohelp and the one
  used on the test system.


